Phase Curves of Kuiper Belt Objects, Centaurs, and Jupiter Family Comets from the ATLAS Survey

The Kuiper belt objects, the Centaurs, and the Jupiter-family comets form an evolutionary continuum of small outer Solar System objects, and their study allows us to gain insight into the history and evolution of the Solar System. Broadband photometry can be used to measure their phase curves, allowing a first-order probe into the surface properties of these objects, though limited telescope time makes measuring accurate phase curves difficult. We make use of serendipitous broadband photometry from the long-baseline, high-cadence ATLAS survey to measure the phase curves for a sample of 18 Kuiper belt objects, Centaurs, and Jupiter-family comets with unprecedentedly large datasets. We find phase curves with previously reported negative slopes become positive with increased data and are thus due to insufficient sampling of the phase curve profile, and not a real physical effect. We search for correlations between phase curve parameters, finding no strong correlations between any parameter pair, consistent with the findings of previous studies. We search for instances of cometary activity in our sample, finding a previously reported outburst by Echeclus and a new epoch of increased activity by Chiron. Applying the main belt asteroid HG1G2 phase curve model to three Jupiter-family comets in our sample with large phase angle spans, we find their slope parameters imply surfaces more consistent with those of carbonaceous main belt asteroids than silicaceous ones.

==> fig10set.tex <==
\figsetstart
\figsetnum{10}
\figsettitle{Phase Curves with $HG1G2$ best fit function overplotted}
\figsetgrpstart
\figsetgrpnum{10.1}
\figsetgrptitle{HG1G2 c filter Hidalgo}
\figsetplot{Phase_Curve_HG1G2_944_Hidalgo_c_Plots_for_Paper.pdf}
\figsetgrpnote{\emph{Left plot:} $HG_{1}G_{2}$ model fit to \emph{c} filter phase curve of (944) Hidalgo. \emph{Right plot:} 2D histogram of Monte Carlo solutions to slope parameters $G_{1}$ and $G_{2}$ of $HG_{1}G_{2}$ fit. Best fit function extended to $\alpha = 0$ deg for ease of viewing any potential opposition surge.}
\figsetgrpnum{10.2}
\figsetgrptitle{HG1G2 o filter Hidalgo}
\figsetplot{Phase_Curve_HG1G2_944_Hidalgo_o_Plots_for_Paper.pdf}
\figsetgrpnote{\emph{Left plot:} $HG_{1}G_{2}$ model fit to \emph{o} filter phase curve of (944) Hidalgo. \emph{Right plot:} 2D histogram of Monte Carlo solutions to slope parameters $G_{1}$ and $G_{2}$ of $HG_{1}G_{2}$ fit. Best fit function extended to $\alpha = 0$ deg for ease of viewing any potential opposition surge.}
\figsetgrpnum{10.3}
\figsetgrptitle{HG1G2 o filter 2014 QA43}
\figsetplot{Phase_Curve_HG1G2_501585_2014_QA43_o_Plots_for_Paper.pdf}
\figsetgrpnote{\emph{Left plot:} $HG_{1}G_{2}$ model fit to \emph{o} filter phase curve of (501585) 2014 QA43. \emph{Right plot:} 2D histogram of Monte Carlo solutions to slope parameters $G_{1}$ and $G_{2}$ of $HG_{1}G_{2}$ fit.}
\figsetgrpnum{10.4}
\figsetgrptitle{HG1G2 o filter Narcissus}
\figsetplot{Phase_Curve_HG1G2_37117_Narcissus_o_Plots_for_Paper.pdf}
\figsetgrpnote{\emph{Left plot:} $HG_{1}G_{2}$ model fit to \emph{o} filter phase curve of (37117) Narcissus. \emph{Right plot:} 2D histogram of Monte Carlo solutions to slope parameters $G_{1}$ and $G_{2}$ of $HG_{1}G_{2}$ fit.}
\figsetgrpend
\figsetend


==> fig4set.tex <==
\figsetstart 
\figsetnum{4}
\figsettitle{Linear fits to phase curves across full phase angle range}
\figsetgrpstart
\figsetgrpnum{4.1}
\figsetgrptitle{Quaoar}
\figsetplot{Phase_Coefficients_50000_Quaoar_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (50000) Quaoar in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.2}
\figsetgrptitle{Hidalgo}
\figsetplot{Phase_Coefficients_944_Hidalgo_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (944) Hidalgo in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}, corrected for rotational modulation. Best fit function extended to $\alpha = 0$ deg for ease of viewing \rcom{the extrapolated absolute magnitude value and} any potential opposition surge.}
\figsetgrpnum{4.3}
\figsetgrptitle{Makemake}
\figsetplot{Phase_Coefficients_136472_Makemake_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (136472) Makemake in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.4}
\figsetgrptitle{Bienor}
\figsetplot{Phase_Coefficients_54598_Bienor_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (54598) Bienor in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.5}
\figsetgrptitle{Chiron}
\figsetplot{Phase_Coefficients_2060_Chiron_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (2060) Chiron in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}, corrected for cometary activity. Best fit function extended to $\alpha = 0$ deg for ease of viewing \rcom{the extrapolated absolute magnitude value and} any potential opposition surge.}
\figsetgrpnum{4.6}
\figsetgrptitle{Chariklo}
\figsetplot{Phase_Coefficients_10199_Chariklo_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (10199) Chariklo in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. Best fit function extended to $\alpha = 0$ deg for ease of viewing \rcom{the extrapolated absolute magnitude value and} any potential opposition surge. }
\figsetgrpnum{4.7}
\figsetgrptitle{Narcissus}
\figsetplot{Phase_Coefficients_37117_Narcissus_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (37117) Narcissus in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.8}
\figsetgrptitle{Huya}
\figsetplot{Phase_Coefficients_38628_Huya_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (38628) Huya in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.9}
\figsetgrptitle{Echeclus}
\figsetplot{Phase_Coefficients_60558_Echeclus_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (60558) Echeclus in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}, corrected for cometary activity. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.10}
\figsetgrptitle{Orcus}
\figsetplot{Phase_Coefficients_90482_Orcus_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (90482) Orcus in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.11}
\figsetgrptitle{Pluto}
\figsetplot{Phase_Coefficients_134340_Pluto_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (134340) Pluto in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}, corrected for rotational modulation. Best fit function extended to $\alpha = 0$ deg for ease of viewing \rcom{the extrapolated absolute magnitude value and} \rcom{the observed} opposition surge\rcom{, most clearly visible in the $o$ filter.}}
\figsetgrpnum{4.12}
\figsetgrptitle{Haumea}
\figsetplot{Phase_Coefficients_136108_Haumea_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (136108) Haumea in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}, corrected for rotational modulation. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.13}
\figsetgrptitle{Eris}
\figsetplot{Phase_Coefficients_136199_Eris_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (136199) Eris in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.14}
\figsetgrptitle{2012 TW236}
\figsetplot{Phase_Coefficients_347449_2012_TW236_Plots_for_Paper.pdf}
\figsetgrpnote{Preliminary linear fit to phase curve of (347449) 2012 TW236 in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.15}
\figsetgrptitle{2009 YF7}
\figsetplot{Phase_Coefficients_349933_2009_YF7_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (349933) 2009 YF7 in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.16}
\figsetgrptitle{2013 XZ8}
\figsetplot{Phase_Coefficients_459865_2013_XZ8_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (459865) 2013 XZ8 in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{4.17}
\figsetgrptitle{2014 QA43}
\figsetplot{Phase_Coefficients_501585_2014_QA43_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of (501585) 2014 QA43 in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. Best fit function extended to $\alpha = 0$ deg for ease of viewing \rcom{the extrapolated absolute magnitude value and} any potential opposition surge.}
\figsetgrpnum{4.18}
\figsetgrptitle{2016 ND21}
\figsetplot{Phase_Coefficients_2016_ND21_Plots_for_Paper.pdf}
\figsetgrpnote{Linear fit to phase curve of 2016 ND21 in ATLAS $o$ and $c$ filters \rcom{for data across the full phase angle range in each filter}. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpend
\figsetend


==> fig7set.tex <==

\figsetstart 
\figsettitle{Linear fits to phase curves across phase angle range $0.1\leq\alpha\leq6$ deg}
\figsetgrpstart
\figsetgrpnum{7.1}
\figsetgrptitle{Quaoar_0_6_deg}
\figsetplot{Phase_Coefficients_50000_Quaoar_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (50000) Quaoar in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.2}
\figsetgrptitle{Makemake_0_6_deg}
\figsetplot{Phase_Coefficients_136472_Makemake_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (136472) Makemake in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.3}
\figsetgrptitle{Bienor_0_6_deg}
\figsetplot{Phase_Coefficients_54598_Bienor_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (54598) Bienor in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.4}
\figsetgrptitle{Chiron_0_6_deg}
\figsetplot{Phase_Coefficients_2060_Chiron_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (2060) Chiron in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg, corrected for cometary activity. Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}
\figsetgrpnum{7.5}
\figsetgrptitle{Chariklo_0_6_deg}
\figsetplot{Phase_Coefficients_10199_Chariklo_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (10199) Chariklo in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge. }
\figsetgrpnum{7.6}
\figsetgrptitle{Huya_0_6_deg}
\figsetplot{Phase_Coefficients_38628_Huya_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (38628) Huya in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.7}
\figsetgrptitle{Echeclus_0_6_deg}
\figsetplot{Phase_Coefficients_60558_Echeclus_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (60558) Echeclus in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg, corrected for cometary activity. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.8}
\figsetgrptitle{Orcus_0_6_deg}
\figsetplot{Phase_Coefficients_90482_Orcus_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (90482) Orcus in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.9}
\figsetgrptitle{Pluto_0_6_deg}
\figsetplot{Phase_Coefficients_134340_Pluto_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (134340) Pluto in ATLAS $o$ and $c$ filters, corrected for rotational modulation. Best fit function extended to $\alpha = 0$ deg for ease of viewing \rcom{the extrapolated absolute magnitude value and the observed} opposition surge\rcom{, most clearly visible in the $o$ filter.}}
\figsetgrpnum{7.10}
\figsetgrptitle{Haumea_0_6_deg}
\figsetplot{Phase_Coefficients_136108_Haumea_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (136108) Haumea in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg, corrected for rotational modulation. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.11}
\figsetgrptitle{Eris_0_6_deg}
\figsetplot{Phase_Coefficients_136199_Eris_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (136199) Eris in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.12}
\figsetgrptitle{2009 YF7_0_6_deg}
\figsetplot{Phase_Coefficients_349933_2009_YF7_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (349933) 2009 YF7 in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpnum{7.13}
\figsetgrptitle{2013 XZ8_0_6_deg}
\figsetplot{Phase_Coefficients_459865_2013_XZ8_Plots_for_Paper_0_6_deg.pdf}
\figsetgrpnote{Linear fit to phase curve of (459865) 2013 XZ8 in ATLAS $o$ and $c$ filters for data in phase angle range $0.1\leq\alpha\leq6$ deg. \rcom{Best fit function extended to $\alpha = 0$ deg for ease of viewing the extrapolated absolute magnitude value and any potential opposition surge.}}
\figsetgrpend
\figsetend

